$\otimes$-Frobenius functors and exact module categories

We call a tensor functor $F:\mathcal{C}\to\mathcal{D}$ between finite tensor categories $\otimes$-Frobenius if its left and right adjoints are isomorphic as $\mathcal{C}$-bimodule functors. We give several characterizations of this notion -- most notably, $F$ is $\otimes$-Frobenius if and only if the centralizer $Z({}_{F}\!{\mathcal{D}}_{\!F})$ is unimodular. We use them to analyze how actions on module categories behave under pullback along $F$. For perfect functors, we show that twisting a $\mathcal{D}$-module category $\mathcal{M}$ along $F$ preserves exactness, and that pivotality, unimodularity, and sphericality are preserved whenever $F$ is $\otimes$-Frobenius (or, more generally, Frobenius with respect to $\mathcal{M}$). Applications include: (i) explicit criteria for $\otimes$-Frobenius functors arising from bialgebra maps $f\!:\!H'\!\to\!H$ between finite-dimensional Hopf algebras; and (ii) criteria ensuring that objects of internal natural transformations are (symmetric) Frobenius algebras in $Z(\mathcal{C})$. Along the way we show that central tensor functors are Frobenius iff they are $\otimes$-Frobenius and that any tensor functor between separable fusion categories is $\otimes$-Frobenius, answering questions of Flake-Laugwitz-Posur.

==> macros.tex <==
\makeatother

%\renewcommand{\baselinestretch}{1.15}
%\onehalfspacing
%\linespread{1.3}

\setlength{\parskip}{1.5pt} 

\setlength\topmargin{0in}
\setlength\headheight{0in}
\setlength\headsep{0.4in}
\setlength\textheight{8.6in}
\setlength\textwidth{6.5in}
\setlength\oddsidemargin{0in}
\setlength\evensidemargin{0in}


\DeclareMathOperator{\rad}{rad}
\DeclareMathOperator{\trace}{trace}
\DeclareMathOperator{\rank}{rank}
\DeclareMathOperator{\charac}{char}
\DeclareMathOperator{\End}{End}
% \DeclareMathOperator{\Ind}{Ind}
\DeclareMathOperator{\Aut}{Aut}
\DeclareMathOperator{\Coind}{Coind}

\newcommand{\Ind}{\mathtt{Ind}}
\newcommand{\bt}{\boxtimes}
\newcommand{\btC}{\bt_{\C}}
\newcommand{\btD}{\bt_{\,\subD}}

\newcommand{\cA}{\mathcal{A}}
\newcommand{\C}{\mathcal{C}}
\newcommand{\B}{\mathcal{B}}
\newcommand{\D}{\mathcal{D}}
\newcommand{\E}{\mathcal{E}}
\newcommand{\X}{\mathcal{X}}
\newcommand{\Y}{\mathcal{Y}}
\newcommand{\Z}{\mathcal{Z}}
\newcommand{\M}{\mathcal{M}}
\newcommand{\N}{\mathcal{N}}
\newcommand{\cL}{\mathcal{L}}
\newcommand{\G}{\mathcal{G}}
\newcommand{\R}{\mathcal{R}}
\newcommand{\YD}{\mathcal{YD}}
\newcommand{\dS}{\mathbb{S}}
\newcommand{\bD}{\mathbf{D}}
\newcommand{\bA}{\mathbf{A}}
\newcommand{\bH}{\mathbf{H}}
\newcommand{\bN}{\mathbf{N}}
\newcommand{\bR}{\mathbf{R}}
\newcommand{\bF}{\textbf{F}}
\newcommand{\bG}{\textbf{G}}
\newcommand{\bc}{\textbf{c}}
\newcommand{\dD}{\mathbb{D}}
\newcommand{\dN}{\mathbb{N}}

\newcommand{\fp}{\mathfrak{p}}
\newcommand{\fq}{\mathfrak{q}}
\newcommand{\fs}{\mathfrak{s}}
\newcommand{\fn}{\mathfrak{n}}
\newcommand{\fu}{\mathfrak{u}}
\newcommand{\fd}{\mathfrak{d}}
\newcommand{\fM}{\mathfrak{M}}
\newcommand{\fR}{\mathfrak{R}}
\newcommand{\fG}{\mathfrak{G}}
\newcommand{\fa}{\mathfrak{a}}
\newcommand{\fb}{\mathfrak{b}}
\newcommand{\fc}{\mathfrak{c}}

\newcommand{\ofn}{\overline{\mathfrak{n}}}
\newcommand{\fnr}{\mathfrak{n}^r}
\newcommand{\fnl}{\mathfrak{n}^l}
\newcommand{\ofs}{\overline{\mathfrak{s}}}

\newcommand{\fsl}{\mathfrak{sl}}

\newcommand{\bi}{\mathbbm{i}}

\newcommand{\zZ}{\mathbb{Z}}

\newcommand{\ff}{\footnote}
\newcommand{\kk}{\Bbbk}
\newcommand{\kkx}{\kk^{\times}}
\newcommand{\ok}{\otimes_{\kk}}
\newcommand{\oL}{\otimes_L}
\newcommand{\oA}{\otimes_A}
\newcommand{\oC}{\otimes_\subC}
\newcommand{\oD}{\otimes_\subD}
\newcommand{\id}{\textnormal{\textsf{Id}}}
\newcommand{\Rep}{\textnormal{\textsf{Rep}}}
\newcommand{\Corep}{\textnormal{\textsf{Corep}}}
\newcommand{\lv}{\hspace{.025cm}{}^{\textnormal{\Scale[0.8]{\vee\!}}} \hspace{-.025cm}}
\newcommand{\rv}{\hspace{.015cm}{}^{\textnormal{\Scale[0.8]{\vee}}} \hspace{-.03cm}}


\newcommand{\Rangle}{\big\rangle}
\newcommand{\Langle}{\big\langle}

\newcommand{\ev}{\textnormal{ev}}
\newcommand{\coev}{\textnormal{coev}}
\newcommand{\VecG}{\textnormal{Vec}_G}
%\newcommand{\Vect}{\operatorname{\text{\usefont{U}{BOONDOX-cal}{m}{n}Vec}}}
\newcommand{\Vect}{\mathsf{Vec}}
\newcommand{\Hom}{\textnormal{Hom}}
\newcommand{\Homk}{\textnormal{Hom}_{\kk}}
\newcommand{\HomL}{\textnormal{Hom}_L}
\newcommand{\HomA}{\textnormal{Hom}_A}
\newcommand{\loc}{\textnormal{loc}}
\newcommand{\co}{\textnormal{co}}

\newcommand{\unit}{\mathds{1}}

\newcommand{\uHom}{\underline{\Hom}}
\newcommand{\uNat}{\textnormal{\underline{Nat}}}
\newcommand{\leftdual}{{}^* \hspace{-.08cm}}
\newcommand{\Hopf}{{\sf Hopf}}
\newcommand{\Alg}{{\sf Alg}}
\newcommand{\Coalg}{{\sf Coalg}}
% \newcommand{\Frob}{{\sf Frob}}
\newcommand{\Bialg}{{\sf Bialg}}
\newcommand{\Rex}{{\sf Rex}}
\newcommand{\Lex}{{\sf Lex}}
\newcommand{\Fun}{{\sf Fun}}
\newcommand{\re}{{\sf re}}
\newcommand{\ra}{{\sf ra}}
\newcommand{\rra}{{\sf rra}}

\newcommand{\la}{{\sf la}}
\newcommand{\lla}{{\sf lla}}
\newcommand{\m}{\mathfrak{m}}
\newcommand{\tr}{{\,{\Act}\,}}
\newcommand{\trF}{\,{{\Act}^{\!\scriptscriptstyle F}}\,}
\newcommand{\tlF}{\,{\triangleleft^{\scriptscriptstyle F}}\,}
\newcommand{\trG}{\,{{\Act}^{\!\scriptscriptstyle G}}\,}
\newcommand{\otr}{\ogreaterthan}
\newcommand{\btr}{\raisebox{0.15ex}{\Scale[0.85]{\blacktriangleright}}}

% \newcommand{\tl}{\,\triangleright\,}

\newcommand{\btl}{\blacktriangleleft}
\newcommand{\tl}{\triangleleft}
\newcommand{\otl}{\olessthan}
\newcommand{\ucoev}{\underline{\textnormal{coev}}}
\newcommand{\ucomp}{\underline{\textnormal{comp}}}
\newcommand{\uev}{\underline{\textnormal{ev}}}
\newcommand{\rev}{\textnormal{rev}}
\newcommand{\op}{\textnormal{op}}
\newcommand{\oop}{\otimes\textnormal{op}}
\newcommand{\mir}{\textnormal{mir}}


\definecolor{darkgreen}{RGB}{55,138,0}
\definecolor{burntorange}{RGB}{180,85,0}
\definecolor{navyblue}{RGB}{18,40,180}
\definecolor{cyan(process)}{rgb}{0.0, 0.6, 1.0}
\newcommand{\red}{\textcolor{red}}
\newcommand{\blue}{\textcolor{navyblue}}
\newcommand{\green}{\textcolor{green}}
\newcommand{\darkgreen}{\textcolor{darkgreen}}
\newcommand{\brown}{\textcolor{brown}}
\newcommand{\gray}{\textcolor{gray}}
\renewcommand{\labelenumi}{(\alph{enumi})}
\renewcommand{\baselinestretch}{1.1}
%-----------------------hyperlinks
\urlstyle{same}


\newcommand{\olive}{\textcolor{olive}}
\newcommand{\thinklater}{\textcolor{magenta}}
\newcommand{\fix}{\textcolor{red}}

\newcommand{\Frob}{{\texorpdfstring{$\otimes$}{}-Frobenius }}
\newcommand{\Frobc}{{$\otimes$-Frobenius,} }
\newcommand{\Frobp}{{$\otimes$-Frobenius.} }

\newcommand{\coFrob}{{dualFrobenius }}
\newcommand{\coFrobc}{{dualFrobenius,} }
\newcommand{\coFrobp}{{dualFrobenius.} }

\newcommand{\tev}{\widetilde{\ev}}
\newcommand{\tcoev}{\widetilde{\coev}}
\newcommand{\ogH}{\overline{\gH}}
\newcommand{\ostar}{\overline{\star}}
\newcommand{\odN}{\overline{\dN}}
\newcommand{\onu}{\overline{\nu}}
\newcommand{\oalpha}{\overline{\alpha}}
\newcommand{\ovarphi}{\overline{\varphi}}
\newcommand{\odD}{{\overline{\dD}}}

\newcommand{\subodD}{{\scriptscriptstyle \odD}}
\newcommand{\subdD}{{\scriptscriptstyle \dD}}

\newcommand{\llb}{\llbracket}
\newcommand{\rrb}{\rrbracket}

\newcommand{\Mod}{\bf Mod}
\newcommand{\moD}{\!\mathrm{mod}}



% \def \trF           {\tr^F\!}

\def\Act           {{\triangleright}}   
\def\act           {\,{\Act}\,}         
\def\Actr          {{\triangleleft}}    
\def\actr          {\,{\Actr}\,}        
\def\actF          {\,{\Yright}\,}
\def\ActrF         {{\Yleft}} 
\def\actrF         {\,\ActrF\,} 
\def\be            {\begin{equation}}
\def\Colon         {:\quad}
\def\DD            {\mathtt{D}}
\def\DDA           {\mathbb{D}_{\Cala}}
\def\dd            {{\rv\rv}}
\def\ldd           {{}{\rv\rv\!}}
\def\ee            {\end{equation}}
\def\Enumerate     {\def\leftmargini{1.34em}~\\[-1.42em]\begin{enumerate}}
\def\Enumeratei    {%\def\leftmargini{1.84em}
	~\\[-1.42em]\begin{enumerate}[{\rm (i)}]\addtolength\itemsep{+1pt}}
\def\Hom           {\mathrm{Hom}}

\def\FD             {{{}_\subF\D}}
\def\FM             {{{}_\subF\M}}
\def\GM             {{{}_\subG\M}}
\def\FN             {{{}_\subF\N}}

\def\id            {{\mathrm{id}}}
\def\Id            {{\mathrm{Id}}}
\def\Im            {{\mathrm{Im}}}
\def\iHom          {\underline{\Hom}}
\def\icoHom          {\underline{\mathrm{coHom}}}
\def\iHomM         {\underline{\Hom}_\calm}
\def\iN            {\,{\in}\,}
\def\iNat          {\underline{\Nat}}
\def\Nat           {\mathrm{Nat}}
\def\opp           {^{\rm opp}}              

\def\PsiN           {{\Psi_{\!\scriptscriptstyle\N}}}
\def\PsiM           {{\Phi_{\!\scriptscriptstyle\M}}}
\def\subFun           {{{\Fun_{\scriptscriptstyle\C}\scriptscriptstyle(\!\M,\scriptscriptstyle\N)}}}
\def \Dag           {{}^\dagger\!}
\def\subF           {{\scriptscriptstyle F}}
\def\subG           {{\scriptscriptstyle G}}
\def\subM           {{\!\scriptscriptstyle \M}}
\def\subFM           {{\!\scriptscriptstyle {\FM}}}
\def\subN           {{\!\scriptscriptstyle \N}}
\def\subC           {{\!\scriptscriptstyle \C}}
\def\subX           {{\!\scriptscriptstyle \X}}
\def\subY           {{\!\scriptscriptstyle \Y}}
\def\subD           {{\!\scriptscriptstyle \D}}
\def\subZ           {{\!\scriptscriptstyle \Z}}
\def\supC           {{\scriptscriptstyle \C}}
\def\supD           {{\scriptscriptstyle \D}}
\def\ot            {\,{\otimes}\,}        
\newcommand{\Se}{\mathbb{S}}              % right Serre functor
\newcommand{\lSe}{\overline{\mathbb{S}}}              % left Serre functor
\def\Xcong         {\xrightarrow{~\cong~}}
\def\xcong         {\,{\Xcong}\,}
\def\xsim         {\,{\xrightarrow{~\sim~}}\,}
\def\xsimeq         {\;{\xrightarrow{~\simeq~}}\;}
\newcommand\rarr[1]{\xrightarrow{~#1~}}
\newcommand\Rarr[1]{\,{\xrightarrow{\,#1\,}}\,}

\def\piv {\mathrm{piv}}
\def\uni {\mathrm{uni}}

\def\ff {\mathsf{f}}
\def\gg {\mathsf{g}}

\newcommand{\gH}{\mathtt{g}_H}
\newcommand{\gHp}{\mathtt{g}_{H'}}
\newcommand{\tnu}{\widetilde{\nu}}
\newcommand{\tg}{\widetilde{\mathsf{g}}}
\newcommand{\ttr}{\tilde{\tr}}
\newcommand{\tG}{\widetilde{G}}
\newcommand{\tfp}{\widetilde{\fp}}
\newcommand{\tfq}{\widetilde{\fq}}
\newcommand{\tfu}{\,\widetilde{\fu}\,}
\newcommand{\tfn}{\widetilde{\fn}}

\def\ZFD{{\Z({}_\subF\D_\subF)}}
\def\FDF{{{}_\subF \D_\subF}}
\def\FDG{{{}_\subF \D_\subG}}
%\def\FD{{{}_\subF\D}}

\def\bchi{\boldsymbol{\chi}}

\newcommand{\chiFf}{\chi_{\scriptscriptstyle F_{\ff}}}
\newcommand{\bg}{\mathbf{g}}
\newcommand{\ba}{\mathbf{a}}
\newcommand{\sa}{\mathtt{a}}
\newcommand{\sg}{\mathtt{g}}
\newcommand{\osg}{\overline{\sg}}


\def \colorComment{purple}
\newcommand{\Change}[1]{\textcolor{\colorComment}{#1}}

